Subgroup Performance of a Commercial Digital Breast Tomosynthesis Model for Breast Cancer Detection

While research has established the potential of AI models for mammography to improve breast cancer screening outcomes, there have not been any detailed subgroup evaluations performed to assess the strengths and weaknesses of commercial models for digital breast tomosynthesis (DBT) imaging. This study presents a granular evaluation of the Lunit INSIGHT DBT model on a large retrospective cohort of 163,449 screening mammography exams from the Emory Breast Imaging Dataset (EMBED). Model performance was evaluated in a binary context with various negative exam types (162,081 exams) compared against screen detected cancers (1,368 exams) as the positive class. The analysis was stratified across demographic, imaging, and pathologic subgroups to identify potential disparities. The model achieved an overall AUC of 0.91 (95% CI: 0.90-0.92) with a precision of 0.08 (95% CI: 0.08-0.08), and a recall of 0.73 (95% CI: 0.71-0.76). Performance was found to be robust across demographics, but cases with non-invasive cancers (AUC: 0.85, 95% CI: 0.83-0.87), calcifications (AUC: 0.80, 95% CI: 0.78-0.82), and dense breast tissue (AUC: 0.90, 95% CI: 0.88-0.91) were associated with significantly lower performance compared to other groups. These results highlight the need for detailed evaluation of model characteristics and vigilance in considering adoption of new tools for clinical deployment.

==> tables/imaging_features_grid_table.tex <==
\begin{figure*}[htbp]
    \centering
    \renewcommand{\arraystretch}{1.2} % Adjust row height for compactness
    \setlength{\tabcolsep}{3pt} % Reduce column spacing
    
    \begin{tabular}{m{2.5cm} m{3cm} m{3cm} m{3cm}} 
        & \centering \textbf{TP} \vspace{4pt} & \centering \textbf{FP} \vspace{4pt} & \centering \textbf{FN} \vspace{4pt} 
        \tabularnewline
        \textbf{Mass} \hspace{5pt} & 
        \includegraphics[width=0.15\textwidth]{figures/imaging_feature/mass/TP/1.2.826.0.1.3680043.8.498.26532128190478886128904655427629823645_frame38_crop.png} &
        \includegraphics[width=0.15\textwidth]{figures/imaging_feature/mass/FP/1.2.826.0.1.3680043.8.498.11469190884689961774128002848437439588_frame29_crop.png} &
        \includegraphics[width=0.15\textwidth]{figures/imaging_feature/mass/FN/1.2.826.0.1.3680043.8.498.15070231600799337806220025282924283329_frame11_crop.png} \tabularnewline
        
        \textbf{Asymmetry} & 
        \includegraphics[width=0.15\textwidth]{figures/imaging_feature/asymmetry/TP/1.2.826.0.1.3680043.8.498.11204901411966165663488437367670442616_frame47_crop.png} &
        \includegraphics[width=0.15\textwidth]{figures/imaging_feature/asymmetry/FP/1.2.826.0.1.3680043.8.498.13147030519313725169381262946230016274_frame23_crop.png} &
        \includegraphics[width=0.15\textwidth]{figures/imaging_feature/asymmetry/FN/1.2.826.0.1.3680043.8.498.11284253127284801979971803628929276392_frame34_crop.png} \tabularnewline
        
        \textbf{Architectural \newline Distortion} & 
        \includegraphics[width=0.15\textwidth]{figures/imaging_feature/arch_distortion/TP/1.2.826.0.1.3680043.8.498.10375644601843260394489785588363784828_frame44_crop.png} &
        \includegraphics[width=0.15\textwidth]{figures/imaging_feature/arch_distortion/FP/1.2.826.0.1.3680043.8.498.12125398858750354639002840194999843999_frame61_crop.png} &
        \includegraphics[width=0.15\textwidth]{figures/imaging_feature/arch_distortion/FN/1.2.826.0.1.3680043.8.498.96134923609102372598920687618214850429_frame29_crop.png} \tabularnewline
        
        \textbf{Calcification} & 
        \includegraphics[width=0.15\textwidth]{figures/imaging_feature/calcification/TP/1.2.826.0.1.3680043.8.498.57107622668031424021715510844681011613_frame24_crop.png} &
        \includegraphics[width=0.15\textwidth]{figures/imaging_feature/calcification/FP/1.2.826.0.1.3680043.8.498.39668374028605568301507408102276409157_frame23_crop.png} &
        \includegraphics[width=0.15\textwidth]{figures/imaging_feature/calcification/FN/1.2.826.0.1.3680043.8.498.10143214251427302986021200032766509038_frame23_crop.png} \tabularnewline
    \end{tabular}
    
    \caption{Examples of model predictions across imaging features of mass, asymmetry, architectural distortion, and calcifications. True positive lesions are from exams containing cancer that were correctly identified by the model. False positive lesions are from cases in which the model predicted cancer for exams that were either deemed negative at diagnostic imaging or benign followings biopsy. False negative lesions are from exams that were malignant on biopsy, however predicted as negative by the model. Note that the model returns only breast-level and exam-level predictions and not regions of interest and these lesions are highlighted (green box) for demonstration purposes. }
    \label{fig:imaging_features_grid}
\end{figure*}
